A data-driven solving strategy based on a greedy optimization algorithm for the analysis of nonlinear beam structures

In the last decade, data-driven computational mechanics (DDCM) has emerged as a novel paradigm in computational mechanics, enabling the direct use of constitutive data - such as stress-strain pairs obtained from experiments, without relying on ad-hoc material models and thereby avoiding information loss. In this work, we extend our data-driven solving strategy GO-ADM, which combines a greedy optimization algorithm with the alternating direction method (ADM), to the structural analysis of geometrically exact beams formulated using director-based kinematics. We discuss a data initialization strategy for nonlinear systems based on a conventional finite element analysis of the same structure using a prescribed constitutive model. The resulting discrete stress and strain fields, possibly obtained under multiple loading scenarios, may also be employed as artificial datasets for the subsequent data-driven computations. Furthermore, we investigate the thermomechanical consistency of both the dataset and the discrete solution, and propose a weak enforcement of this consistency in the latter via a penalty approach. Numerical examples involving single- and multi-member structures demonstrate that the proposed penalty term leads to thermomechanically consistent discrete stress and strain fields. Moreover, for the studied examples, the solving strategy GO-ADM yields a generally improved approximation of the globally optimal solution compared to the standard ADM-based direct solver.

==> algorithms/localstateassigment.tex <==
\begin{algorithm}[h]
\textbf{Input}:
	solution $\qhat$, 
    dataset $\dataset$ \\
\textbf{Output}: $\ytilde$
\begin{algorithmic}[1]
    \State Collect $\yhat = \left(\hat{\vect{e}},\, \hat{\vect{s}}\right)$ from $\qhat$
    \For{$i$ in $1,\ldots,\mdofs$}
        \State Choose $\ytilde_i \in \dataset$ s.t. 
        $\eleObjFunc \left(\yhat,\,\ytilde_i\right)$ = min.       \Comment{See also Equation \eqref{eq:eleObjectiveFunc}}
    \EndFor
    \State Return $\ytilde$
\caption{Local state assignment: selection of the stress--strain pairs $\ytilde \in \dataset$ that are closest to $\yhat$.}\label{alg:localstateassigment}
\end{algorithmic}
\end{algorithm}
    
